A Model Structure On The Category Of Small Acyclic Categories

In this paper, we show that the Thomason model structure restricts to a Quillen equivalent cofibrantly generated model structure on the category of acyclic categories, whose generating cofibrations are the same as those generating the Thomason model structure. To understand the Thomason model structure, we need to have a closer look at the (barycentric) subdivision endofunctor on the category of simplicial sets. This functor has a well known right adjoint, called Kan's Ex functor. Taking the subdivision twice and then the fundamental category yields a left adjoint of an adjunction between the category of simplicial sets and the category of small categories, whose right adjoint is given by applying the Ex functor twice on the nerve of a category. This adjunction lifts the cofibrantly generated Quillen model structure on simplicial sets to a cofibrantly generated model structure on the category of small categories, the Thomason model structure. The generating sets are given by the image of the generating sets of the Quillen model structure on simplicial sets under the aforementioned adjunction. We furthermore show that the category of acyclic categories is proper and combinatorial with respect to said model structure. That is weak equivalences behave nicely with respect to pushouts along fibrations and cofibrations, and cofibrations satisfy certain smallness conditions which allow us to work with sets instead of proper classes.

==> abstract.tex <==
\begin{abstract}
A 2-category generalizes the concept of a category by adding 2-morphisms between arrows. The easiest example would be the category of small categories, with functors between categories as the usual morphisms, and natural equivalences between functors as 2-morphisms. One can weaken the notion of a 2-category to a weak 2-category. That is, the unit and associativity laws for concatenation of arrows are only required to hold up to 2-morphisms.\\
An  example for a weak 2-category is the correspondence 2-category $\Corr(2)$, which consist of $C^*$-algebras as objects, $C^*$-correspondences as morphisms and $C^*$-correspondence isomorphisms as 2-morphisms. Since invertible $C^*$-corres- \newline pondences are imprimitivity bimodules, isomorphisms in $\Corr(2)$ become Morita equivalences.\\
Given an arbitrary weak 2-category, one can define weak actions of groups, 2-groups, groupoids or 2-groupoids on objects in the given category as 2-functors. That is, given one of the former mentioned structures, every property of the action is already encoded in the definition of the 2-functor.\\
Now given a weak group action $(A,\alpha,\omega, u)$ of a discrete group $G$ on a $C^*$-algebra $A$ in $\Corr(2)$, Buss, Zhu and Meyer have proved in \cite{highcatapp} that this is equivalent to a Fell Bundle $\bundle{A}$ over $G$, together with an isomorphism $\phi\colon A_e\to A$, where $A_e$ denotes the unitfiber.\\
To achieve this, one can view any fiber $A_g$ in $\bundle{A}$ as an $A_e$-$A_e$ bimodule, and by defining some inner products $\lind{A_e}\iprod{a_g}{b_g} := a_g^*b_g$ respectively $\iprod{a_g}{b_g}_{A_e} := a_gb_g^*$ these become even $A_e-A_e$-imprimitivity bimodules. By defining $\alpha_g := A_{g^{-1}}$ these yield a weak group action by $C^*$-correspondences.\\
Conversely, given a weak group action one defines the fibers of the Fell bundle via $A_g := \alpha_{g^{-1}}$. The only problem is finding the right involution on $\bundle{A}$, which is solved by taking the (unique) dual of a given $A-A$-imprimitivity bimodule $\alpha_g = A_{g^{-1}}$.\\
This construction can be generalized to topological groups. Therefore, one can see any weak group action by $C^*$-correspondences as an upper semi continuous bundle of imprimitivity bimodules. Then continuity can be expressed in terms of sections.\\
Going from discrete groups to r-discrete groupoids is rather canonical, and it is easy to see that weak group actions by $C^*$-correspondences are equivalent to some Fell bundle over an r-discrete groupoid.\\
More interesting is the step from groups to 2-groups. It is well known, that any 2-group is equivalent to a crossed module. Moreover, a crossed module can be seen as a generalization of a quotient group. There is a theorem by Echterhoff and Quigg \cite[Theorem~5.1]{echt:indcoac}, stating that given a discrete group $G$, a normal subgroup $N\subset G$, a quotient map $q\colon G\to G/N$, and a Fell bundle $\bundle{B}$ over $G/N$, a Fell bundle $\bundle{A}$ over $G$ is isomorphic to the pull-back bundle $q^*\bundle{B}$, iff there is a homomorphism $u$ from $N$ into $\mathcal{UM}(A)$, such that 
	\begin{enumerate}
		\item $u_n\in\mathcal{UM}(\bundle{A})_n$ for all $n\in  N$, and
		\item $a_su_n = u_{sns^{-1}}$ for all $a_s\in A_s$, $n\in N$.
	\end{enumerate}
One can use this, to find a definition of a Fell bundle over a crossed module, hence a 2-group, by saying a Fell bundle $\bundle{A}$ over some crossed module $\mathcal{C} = (G,H,\partial,\gamma)$ is an ordinary Fell bundle over $G$, together with an homomorphism $H\colon\mathcal{UM}(A)$, such that 
	\begin{enumerate}
			\item $u_h\in\mathcal{UM}(\mathcal{A})_{\partial(h)}$ for all $h\in H$
			\item $a\cdot u_h = u_{\gamma_g(h)}\cdot a$ for all $a\in A_g$, $h\in H$.
	\end{enumerate}
It is possible to show, that using this definition, a weak 2-group action by $C^*$-correspondences of a discrete 2-group $G$ on a $C^*$-algebra $A$ is equivalent to a Fell bundle over a discrete crossed module.\\
Again, this can be generalized to topological 2-groups by defining continuity of a 2-group action in terms of sections (and using some canonical continuity assumptions on the Fell bundle).\\
Finally, combining any further results, it is easy to see that one can even find an equivalence between weak actions of r-discrete 2-groupoids by $C^*$-correspondences and Fell bundles over r-discrete 2-groupoids.

\end{abstract}

